Face2Face: Real-time Face Capture and Reenactment of RGB Videos

We present Face2Face, a novel approach for real-time facial reenactment of a monocular target video sequence (e.g., Youtube video). The source sequence is also a monocular video stream, captured live with a commodity webcam. Our goal is to animate the facial expressions of the target video by a source actor and re-render the manipulated output video in a photo-realistic fashion. To this end, we first address the under-constrained problem of facial identity recovery from monocular video by non-rigid model-based bundling. At run time, we track facial expressions of both source and target video using a dense photometric consistency measure. Reenactment is then achieved by fast and efficient deformation transfer between source and target. The mouth interior that best matches the re-targeted expression is retrieved from the target sequence and warped to produce an accurate fit. Finally, we convincingly re-render the synthesized target face on top of the corresponding video stream such that it seamlessly blends with the real-world illumination. We demonstrate our method in a live setup, where Youtube videos are reenacted in real time.

==> 3overview.tex <==
\section{Overview}
\label{sec::overview}

\begin{figure}
	\centering
	\ifdefined\LOWRES
	\includegraphics[width=0.9\linewidth]{images/pipeline2.jpg}
	\else
	\includegraphics[width=0.9\linewidth]{images/pipeline2}
	\fi
	\caption{Method overview.}
	\label{fig":overview}
\end{figure}


%
In the following, we describe our real-time facial reenactment pipeline (see Fig.~\ref{fig::overview}).
%
Input to our method is a monocular target video sequence and a live video stream captured by a commodity webcam.
%
First, we describe how we synthesize facial imagery using a statistical prior and an image formation model (see Sec.~\ref{sec::synthesis}).
%
We find optimal parameters that best explain the input observations as a robust variational energy minimization problem (see Sec.~\ref{sec::energy}).
%
We minimize this energy with a tailored, data-parallel GPU-based \textit{Iteratively Reweighted Least Squares} (IRLS) solver (see Sec.~\ref{sec::optimization}).
%
We employ IRLS for offline non-rigid model-based bundling (see Sec.~\ref{sec::bundling}) on a set of selected keyframes to obtain the facial identity of the source as well as of the target actor.
%
This step jointly recovers the facial identity, expression, skin reflectance, and illumination from monocular input data.
%
At runtime, both source and target animations are reconstructed based on a model-to-frame tracking strategy with a similar energy formulation.
%
For reenactment, we propose a fast and efficient deformation transfer approach that directly operates in the subspace spanned by the used statistical prior (see Sec.~\ref{sec::transfer}).
%
The mouth interior that best matches the re-targeted expression is retrieved from the input target sequence (see Sec.~\ref{sec::mouth}) and is warped to produce an accurate fit.
%
We demonstrate our complete pipeline in a live reenactment setup that enables to modify arbitrary video footage and compare to state-of-the-art tracking as well as reenactment approaches (see Sec.~\ref{sec::results}).
%
Finally, we conclude with an outlook on future work (see Sec.~\ref{sec::conclusion}).

